Parallel Maximum Clique Algorithms with Applications to Network Analysis and Storage

We propose a fast, parallel maximum clique algorithm for large sparse graphs that is designed to exploit characteristics of social and information networks. The method exhibits a roughly linear runtime scaling over real-world networks ranging from 1000 to 100 million nodes. In a test on a social network with 1.8 billion edges, the algorithm finds the largest clique in about 20 minutes. Our method employs a branch and bound strategy with novel and aggressive pruning techniques. For instance, we use the core number of a vertex in combination with a good heuristic clique finder to efficiently remove the vast majority of the search space. In addition, we parallelize the exploration of the search tree. During the search, processes immediately communicate changes to upper and lower bounds on the size of maximum clique, which occasionally results in a super-linear speedup because vertices with large search spaces can be pruned by other processes. We apply the algorithm to two problems: to compute temporal strong components and to compress graphs.

==> sec-compression.tex <==

\def \imgcompsz {0.9\linewidth}


\begin{figure}[b!]
\vspace{-2mm}
\centering
\hspace{-6ex}
\label{fig:comp-penn}\includegraphics[width=\imgcompsz]{pmc-compression/comp-sm} 
\vspace{-2mm}
  \caption{\textbf{Compression via clique-based ordering}. 
  The figure compares three sizes of a graph: the original graph $G$, a compression of $G$ using the
  BV method based on the native ordering or vertices (bvgraph), and a similar compression based
  on clique-based ordering (pmc-heu).  
  In pmc-heu, vertices inside each clique are ordered by degree. 
  %Note that degenercy ordering also gave similar results and were removed due to brevity.
  }
\label{fig:pmc-compression}
\vspace{-4mm}
\end{figure}



%labels{1} = 'original';
%labels{2} = 'bvgraph';
%labels{3} = 'pmc-heu';
%
%    18384092     4237507     3104286
%    21333870     4605427     3508224
%
%    1.0000    0.2305    0.1689
%    1.0000    0.2159    0.1644



\section{Graph Compression}
\label{sec:compress}

Graph compression saves storage space and improves the runtimes of algorithms.
Both are especially important for computations over big graphs.
Recently, ...\cite{kang2011beyond,boldi2011layered}.

In methods such as \cite{boldi2011layered}, one can expect to improve compression by
using an ordering of vertices in a network that brings as many of the nodes of the network 
along the block diagonal of the adjacency matrix representation of the network.
To that end we obtain such an ordering by repeatedly applying our maximum clique algorithm
to a network. In particular, given a graph $G$, we find a maximum clique $C$ in $G$, remove $C$
from $G$, and repeat the process until all vertices are removed. We then order the vertices according to the
cliques, $C_1$, $C_2$, $\ldots$, $C_K$, where $K$ denotes the number of iterations needed.
Internally within each $C_i$ we order the vertices by their degrees.
We feed the compression method from \cite{boldi2011layered} with such an ordering.
Figure~\ref{fig:pmc-compression} shows the results we get on two Facebook networks 
(FB-Penn State and FB-Texas from Table 1).
It can be seen that the ordering results in better compression compared to a native ordering.
Figure~\ref{fig:adj-clique-order}, which shows a spy-plot of  a portion of the adjacency matrix of the
two Facebook networks with native ordering and clique-based ordering, explains why the reordering
results in improved compression. 

To reduce runtime needs we used in the reordering cliques computed by our heuristic,
instead of the exact algorithm.
 
 


%\begin{Definition}[Clique Ordering Problem]
%Given a graph $G=(V,E)$, 
%an ordering $P$ is a maximum clique ordering if and only if $P = \{C_{1},C_{2},...,C_{k}\}$
%where $C_{1},C_{2},...,C_{k}$ are the set of maximum cliques from the graphs $G, G(V-C_1), ..., G(V - [C_1 \cup C_2 \cup \cdots \cup C_k])$ such that $|C_1| \geq |C_2| \geq \cdots \geq |C_k|$.
%The clique ordering problem is to find such an ordering. 
%\end{Definition}


%The \textit{clique ordering} is computed iteratively using a few basic steps:
%Consider the simple through a few simple intuitive steps:
%\begin{compactenum}[1.]
%\item Find a maximum clique $C$
%\item Remove $C$ from the graph $G$
%\item Repeat until all vertices are removed
%\end{compactenum}


%We develop heuristic and exact clique ordering methods.
%The heuristic method is extremely fast but results in slightly less compression, whereas the exact clique ordering takes longer, but results in slightly better compression.

%Observe that the order in which the maximum cliques are removed effects the solutions in the future iterations.
%Moreover, there is no guarantee that the same maximum cliques will be found in two subsequent runs due to the non-deterministic nature of the parallel algorithm.
%In the future, we plan to reorder the cliques themselves by greedily merging the ones that maximize some objective.


%The selection of the algorithm depends on the graph and thus our data-driven algorithm optimizer can be used.

%Heuristic is extremely fast but less accurate and exact is still fast, but more accurate.
%Each has advantages and disadvantages over the other which are summarized in the Table~\ref{table:clique-ordering}.
%Note the term class is used here, since any of the algorithms from the pmc framework (see Table~\ref{table:pmc-framework}) may be used for each of the classes.
%In addition, any heuristic and exact maximum clique algorithm from the pmc framework may be used here.
%The algorithm is selected by data-driven optimization




%\textbf{Heuristic}.
%For the heuristic maximum clique ordering, there are only a few differences: 
%(1) the function $C = $\textsc{ParallelMC}$(G,K,lb)$ is only used in the first iteration, and
%(2) in the subsequent iterations, the function \textsc{Heuristic}$(G,K)$ returns a large clique $C$, which is then removed.

%The intuition of finding the exact maximum clique is to 

%\algrenewcommand{\alglinenumber}[1]{\scriptsize #1}
%\begin{algorithm}[H]
%\vspace{-0mm}
%\caption{Simple Algorithm for Maximum Clique Ordering}
%\label{alg:clique-ordering}
%{
%\scriptsize
%\begin{algorithmic}[1]
%\State \textbf{Input:} $G=\left (V,E\right )$ -- a graph
%\State \quad \quad \quad \quad $\delta$ -- stopping criterion for smallest clique
%\State \textbf{Output:} $P$ -- vertices ordered by maximum clique  %an ordered set of vertices
%
%\Repeat
%\State $C = \emptyset$
%\State $K = CoreNumbers(G)$
%%\State $C_heu = Heuristic(G,K)$ % Find a large clique $C$ in $G$ using heuristic
%%\State $lb = |C_{heu}|$
%\State $lb = $\textsc{Heuristic}$(G,K)$ % Find a large clique $C$ in $G$ using heuristic
%\State $C = $\textsc{ParallelMC}$(G,K,lb)$
%\State Order $C$ by degree (or cores)
%\State Add vertices in $C$ to the back of $P$ in order
%\State Set $G = (W,E[W])$, where $W = V - C$ %% = \{u : u \in V \text{and} u \not\in C \}$
%\State $V = W$
%\Until{$V = \emptyset$ or $|C| < \delta$} %or $V = \emptyset$
%
%\State Compute degree or cores for remaining vertices
%\State Order remaining vertices by degree (or kcore)
%\State Add ordered vertices to $P$
%\end{algorithmic}}
%\end{algorithm}




\def \adjsz {0.45\linewidth}

\begin{figure}[t!]
\vspace{-2mm}
\centering
      	\subfigure[fb-Penn (initial)]
    			{\hspace{-2ex}\label{fig:adj-cmu-exact-deg}\includegraphics[width=\adjsz]
    			{pmc-compression/adj-socfb-Penn94-exact-deg-500-prev}}   	
     	\subfigure[fb-Penn (clique-based reordering)]
    			{\hspace{-2ex}\label{fig:adj-cmu-exact-deg}\includegraphics[width=\adjsz]
    			{pmc-compression/adj-socfb-Penn94-exact-deg-500}}  
    			\vspace{-4mm}
     	\subfigure[fb-Texas (initial)]
    			{\vspace{-4mm}\hspace{-2ex}\label{fig:adj-cmu-exact-deg}\includegraphics[width=\adjsz]
    			{pmc-compression/adj-socfb-Texas-exact-deg-500-prev}}   	
     	\subfigure[fb-Texas (clique-based reordering)]
    			{\hspace{-2ex}\label{fig:adj-cmu-exact-deg}\includegraphics[width=\adjsz]
    			{pmc-compression/adj-socfb-Texas-exact-deg-500}} 	 
\caption{Nonzero structure of adjacency matrix with native (initial) ordering and a reordering based on maximum cliques.}
%The maximum clique ordering is shown on the right compared to the initial ordering on the left.}
\label{fig:adj-clique-order}
\vspace{-4mm}
\end{figure}







%\def \compimgsz {2.0in}%{0.24\linewidth}
%
%\begin{figure*}[t]
%\vspace{-2mm}
%\centering
%\subfigure[Bounds (exact)]
%{\hspace{-2ex}\label{fig:adj-cmu-exact-deg}\includegraphics[width=\compimgsz]
%{pmc-compression/bounds-socfb-CMU-exact-deg}} 
%\subfigure[Time]
%{\hspace{-2ex}\label{fig:adj-texas-exact-deg}\includegraphics[width=\compimgsz]
%{pmc-compression/methods-time-socfb-CMU}}  
%\subfigure[Clique size]
%{\hspace{-2ex}\label{fig:adj-texas-exact-deg}\includegraphics[width=\compimgsz]
%{pmc-compression/methods-clique-socfb-CMU}}  
%		
%\caption{}
%%\textbf{Time vs Iteration}.
%%  For each graph, we compare against four variants of the clique ordering.
%%  We observe that the runtime decreases as the clique size decreases.
%%  We also see that the heuristic algorithm is 2-3 times faster than the exact.
%% Further, the heuristic shows a stable decrease in runtime, whereas a few of the the exact algorithm iterations increase. 
%\label{fig:pp-plots}
%\vspace{-4mm}
%\end{figure*}









%
%\def \boundsimgszcomp {0.44\linewidth}
%
%\begin{figure}[t]
%\vspace{-2mm}
%\centering
%
%\subfigure[MIT (exact)]
%{\hspace{-2ex}\label{fig:adj-cmu-exact-deg}\includegraphics[width=\boundsimgszcomp]
%{pmc-compression/bounds-socfb-MIT-exact-deg}}   
%%   			
%%\subfigure[MIT (heu)]
%%{\hspace{-2ex}\label{fig:adj-texas-exact-deg}\includegraphics[width=\boundsimgszcomp]
%%{pmc-compression/bounds-socfb-MIT-heu-deg}}  
%%%
%\subfigure[CMU (exact)]
%{\hspace{-2ex}\label{fig:adj-cmu-exact-deg}\includegraphics[width=\boundsimgszcomp]
%{pmc-compression/bounds-socfb-CMU-exact-deg}}   
%% 			
%%\subfigure[CMU (heu)]
%%{\hspace{-2ex}\label{fig:adj-texas-exact-deg}\includegraphics[width=\boundsimgszcomp]
%%{pmc-compression/bounds-socfb-CMU-heu-deg}}  
%%
%\subfigure[Penn (exact)]
%{\hspace{-2ex}\label{fig:adj-cmu-exact-deg}\includegraphics[width=\boundsimgszcomp]
%{pmc-compression/bounds-socfb-Penn94-exact-deg}}   
%%			
%%\subfigure[Penn (heu)]
%%{\hspace{-2ex}\label{fig:adj-cmu-exact-deg}\includegraphics[width=\boundsimgszcomp]
%%{pmc-compression/bounds-socfb-Penn94-heu-deg}}  
%%
%\subfigure[Texas (exact)]
%{\hspace{-2ex}\label{fig:adj-cmu-exact-deg}\includegraphics[width=\boundsimgszcomp]
%{pmc-compression/bounds-socfb-Texas-exact-deg}}   
%%	
%%\subfigure[Texas (heu)]
%%{\hspace{-2ex}\label{fig:adj-texas-exact-deg}\includegraphics[width=\boundsimgszcomp]
%%{pmc-compression/bounds-socfb-Texas-heu-deg}}  
%    			
%  \caption{}
%\label{fig:pp-plots}
%\vspace{-4mm}
%\end{figure}
%



%
%
%\def \compimgsz {2.6in}%{0.24\linewidth}
%
%\begin{figure}[t]
%\vspace{-2mm}
%\centering
%
%\subfigure[MIT]
%{\hspace{-2ex}\label{fig:adj-cmu-exact-deg}\includegraphics[width=\compimgsz]
%{pmc-compression/methods-clique-socfb-MIT}}   
%%
%\subfigure[CMU]
%{\hspace{-2ex}\label{fig:adj-texas-exact-deg}\includegraphics[width=\compimgsz]
%{pmc-compression/methods-clique-socfb-CMU}}  
%%
%\subfigure[Penn]
%{\hspace{-2ex}\label{fig:adj-cmu-exact-deg}\includegraphics[width=\compimgsz]
%{pmc-compression/methods-clique-socfb-Penn94}}   
%%   			
%\subfigure[Texas]
%{\hspace{-2ex}\label{fig:adj-texas-exact-deg}\includegraphics[width=\compimgsz]
%{pmc-compression/methods-clique-socfb-Texas}}  
%		
%\caption{\textbf{Clique size vs Iteration}.
%  For each graph, we compare against four variants of the clique ordering.
%  }
%\label{fig:pp-plots}
%\vspace{-4mm}
%\end{figure}
%
%
%sz = [
%      406326      407317      407383      408775      543590;
%      405698      405815      406711      407593      535974;
%     3092729     3101178     3104286     3114471     4237507;
%     3497973     3504101     3508224     3512659     4605427;
%];


==> sec-tscc.tex <==


%\section{Applications}
%In section~\ref{sec:data}, we used our parallel maximum clique finder to understand the behavior of a variety of networks.
%Here, we demonstrate the effectiveness of our algorithms for finding temporal strong components and improving graph compression.
%exploratory analysis on a variety of networks.


\section{Temporal Strong Components} 
\label{sec:tscc}

In this section, we use the maximum clique method as a subroutine to compute temporal strong components~\cite{bhadra2003complexity,nicosia:023101}.  
Since this area is somewhat new, we review some of the basic definitions in order to motivate the relationship between cliques and temporal strong components.
%\vspace{-0.5ex} \begin{Definition}[temporal network]
Let $V$ be a set of vertices, and $E_T \subseteq V \times V \times \RR^{+}$ be the set of temporal edges between vertices in $V$. Each edge $(u,v,t)$ has a unique time $t \in \RR^{+}$.
%\end{Definition} \vspace{-0.5ex}
For such a temporal network, a path represents a sequence of edges that must be traversed in increasing order of edge times.  That is, if each edge represents a contact between two entities, then a path is a feasible route for information.
\begin{Definition}[temporal paths]
A temporal path from $u$ to $w$ in $G=(V,E_T)$ is a sequence of edges $e_1, \ldots, e_k$ such that the $e_1\!=\!(u,v_1,t_1), \ldots, e_k\!=\!(u_k, w, t_k)$ where $v_{j} = u_{j+1}$ and $t_j < t_{j+1}$ for all $j = 1$ to $k$.
We say that $u$ is \textit{temporally connected} to $w$ if there is such a temporal path.
\end{Definition}
This definition echoes the standard definition of a path, but adds the additional constraint that paths must follow the directionality of time.
Temporal paths are inherently asymmetric because of the directionality of time.

\def \lentab{2.5in}
\begin{figure}[t!]
\centering
    \hspace{-2mm}\subfigure[Reachability (retweet)]
    	{\label{fig:reach-retweets}\includegraphics[width=0.5\linewidth]{images/retweet-2parties-Rs-sm.png}}
    \subfigure[Temporal SCC (retweet)]
    	{\label{fig:tscc-retweets}\includegraphics[width=0.5\linewidth]{images/retweet-pol-scc-sm.png}}
    	\vspace{-3mm}    	
  \caption{In order to compute the largest temporal strong component, we first compute the strong reachability network (a). These networks are rather dense and often reveal clear community structure. Here we see clear communities for the political left and right.  We find that the largest temporal strong component in the retweet network (b) consists of 166 twitter users classified as politically ``right'' according to the original data with only a single exception. }
  \label{fig:tscc-vis}
  \vspace{-3mm}
\end{figure}


\begin{Definition}[temporal strong component]
Two vertices $(u,w)$ are strongly connected if there exists a temporal path $\mathcal{P}$ from $u$ to $w$ and from $w$ to $u$.  A temporal strongly connected component (tSCC) is defined as a maximal set of vertices $C \subseteq V$ such that any pair of vertices in $C$ are strongly connected.
\end{Definition}
While the vertices of a strong component in a graph define an equivalency class, and hence, we can partition a network into components, the same fact is not true of temporal strong components.  The vertices in a temporal strong component can overlap with those in another temporal strong component.
%Note that a temporal weak component is always equal to the connected component in the static graph~\cite{tang2010characterising}.  We conclude by mentioning that stronger definitions of temporal components exist.  For example, the temporal paths used to define a strong component can be further restricted to only use vertices from the component $C$ itself.
As previously mentioned, checking if a graph has a $k$-node temporal SCC is NP-complete~\cite{bhadra2003complexity,nicosia:023101}.  Nonetheless, we can compute the largest such strong component using a maximum clique algorithm.  Let us briefly explain how.  

The first step is to transform the temporal graph into what is called a strong-reachability graph.  For each pair of vertices in $V$, we place an edge in the strong reachability graph if there is a temporal path between them.  In Algorithm~\ref{alg:tscc}, this corresponds to the \textsc{reach} subroutine.  That method uses the temporal ordering proposed by~\cite{Pan-2011-paths} and builds up temporal paths backwards in time. With this reachability graph, the second step of the computation is to remove any non-reciprocated edges and then find a maximum clique.  That maximum clique is the largest set of nodes where all pairwise temporal paths exist, and hence, is the largest temporal strong component~\cite{nicosia:023101}.


\input{alg-reach}


%
%\subsection{Temporal Graph Data.}
%\label{sec:tscc-data}
%
%We use four types of temporal graph data.  For all networks, we discard self-loops and any edge weights.  In all cases, the nodes represent people.  And in all cases, the largest temporal strong components reflect groups of people that meet, interact, or retweet with each other sufficiently often to transmit any message or meme.
%
%\begin{compactenum}[1.]
%\item \textbf{Contact networks}.
%The edges are face-to-face contacts (infect-dublin, infect-hyper\cite{isella2011s}). See ref.~\cite{infect} for more details about these data.
%
%
%\item \textbf{Interaction networks}.
%The edges are observed interactions such as forum posts (fb-forum~\cite{opsahl2011triadic}), private messages (fb-messages~\cite{opsahl2009clustering}), or emails (enron~\cite{cohen2005enron}).
%We also investigate a cellular telephone call network where the edges are calls (reality~\cite{eagle2006reality}). 
%
%\item \textbf{Retweet networks}.
%Here, the edges are retweets. We analyzed a network of political retweets centered around the November 2010 election in the US (retweet~\cite{conover2011political}).
%A similar dataset is a retweet and mentions network from the UN conference held in Copenhagen. The data was collected over a two week period (twitter-copen~\cite{ahmed2010time}).  
%
%\item \textbf{Hashtag networks}.
%Again the edges are retweets associated with a hashtag. We collected these from Truthy~\cite{truthy} on September 20th, 2012.  Of these, only a few had non-trivial temporal strong components which we discuss below.
%\end{compactenum}
%

%infectious
%\textbf{Contact networks}.
%The edges are face-to-face contacts (infect-dublin, infect-hyper\cite{isella2011s}). See ref.~\cite{infect} for more details about these data.
%
%
%\textbf{Interaction networks}.
%The edges are observed interactions such as forum posts (fb-forum~\cite{opsahl2011triadic}), private messages (fb-messages~\cite{opsahl2009clustering}), or emails (enron~\cite{cohen2005enron}).
%We also investigate a cellular telephone call network where the edges are calls (reality~\cite{eagle2006reality}). 
%
%\textbf{Retweet networks}.
%Here, the edges are retweets. We analyzed a network of political retweets centered around the November 2010 election in the US (retweet~\cite{conover2011political}).
%A similar dataset is a retweet and mentions network from the UN conference held in Copenhagen. The data was collected over a two week period (twitter-copen~\cite{ahmed2010time}).  
%
%\textbf{Hashtag networks}.
%Again the edges are retweets associated with a hashtag. We collected these from Truthy~\cite{truthy} on September 20th, 2012.  Of these, only a few had non-trivial temporal strong components which we discuss below.

\begin{table}[t!]
%TODO: Remove large text from table captions, it is strongcaps
\caption{For each temporal network, we list the number of temporal edges, the number of vertices and edges in the reachability graph, the size $\omega$ of the temporal strong component and the runtime of our algorithm.}
\vspace{1mm}
%max clique in the reachability graph  (the size of the temporal strong component), and the time to compute the max clique.}
%
\label{table:tscc}
\centering
%\small %ted
\scriptsize
\begin{tabularx}{0.85\linewidth}{@{}rXXXHHHXcHH@{}}
\toprule 
\textbf{graph} & $|E_{T}|$ & $|V_{R}|$ & $|E_{R}|$ & $K$ & $\tilde{\omega}$ & $\mu$ & $\omega$ & Time \rlap{(s.)} & $\tau_{heu}$ & $\tau_{\mu}$\\ 
\midrule 
 \textsc{infect}-\textsc{dublin} & 415k & 11k & 176k & 84 & 84 & 1 & 84 & $<$.01 & 1 & 3.38\\ 
 \textsc{infect}-\textsc{hyper} & 20k & 113 & 6.2k & 106 & 106 & 1 & 106 & $<$.01 & 1 & 4.45\\ 
 \midrule
% \textsc{enron} & 50k & 151 & 9.8k & 120 & 120 & 2 & 120 & $<$.01 & 1 & 8.19\\ 
% \textsc{fb}-\textsc{forum} & 33k & 897 & 71k & 273 & 266 & 1 & 266 & 0.02 & 0.74 & 1.34\\ 
 \textsc{fb}-\textsc{messages} & 61k & 1.9k & 532k & 707 & 707 & 3 & 707 & 0.05 & 1 & 3.95\\ 
 \textsc{reality} & 52k & 6.8k & 4.7M & 1236 & 1236 & 1 & 1236 & 0.19 & 1 & 4.8\\ 
 \midrule
 \textsc{retweet} & 61k & 18k & 66k & 175 & 165 & 1 & 166 & 0.02 & 0.48 & 1.41\\ 
 \textsc{twitter}-\textsc{cop} & 45k & 8.6k & 474k & 583 & 581 & 1 & 581 & 0.22 & 0.55 & 1.44\\ 
%\midrule 
% \textsc{mittromney} & 8.5k & 7.8k & 108 & 5 & 5 & 5 & 5 & $<$.01 & 1 & 28.36\\ 
% \textsc{bahrain} & 8k & 4.7k & 129 & 8 & 8 & 2 & 8 & $<$.01 & 1 & 31.85\\ 
% \textsc{barackobam} & 9.8k & 9.6k & 226 & 10 & 10 & 3 & 10 & $<$.01 & 1 & 56.13\\ 
% \textsc{alwefaq} & 7.1k & 4.2k & 355 & 16 & 16 & 3 & 16 & $<$.01 & 1 & 24.5\\ 
% \textsc{justinbieb} & 9.6k & 9.4k & 442 & 17 & 17 & 2 & 17 & $<$.01 & 1 & 68.81\\ 
% \textsc{occupywall} & 3.9k & 3.6k & 931 & 18 & 18 & 4 & 18 & $<$.01 & 1 & 52.56\\ 
% \textsc{gmanews} & 8.8k & 8.3k & 1.1k & 22 & 22 & 2 & 22 & $<$.01 & 1 & 63.4\\ 
% \textsc{lolgop} & 10k & 9.7k & 4.5k & 42 & 42 & 2 & 42 & $<$.01 & 1 & 35.55\\ 
\midrule 
\end{tabularx}
\vspace{-4mm}
\end{table}



%\subsection{Results and analysis}
\noindent \textbf{Results and analysis}.
Figure~\ref{fig:tscc-vis} shows the reachability and largest temporal strong component from the retweet network about politics.  It took the maximum clique finder less than a second to identify this clique.  We summarize the remaining experiments on the temporal strong components in Table~\ref{table:tscc}.  For all of these networks, we were able to identify the largest temporal strong component in less than a second after we computed the reachability network. There are two reasons for this performance.  First, in all of the networks except for the interaction networks, the largest clique is the set of vertices with highest core numbers.  Second, our heuristic computes the largest clique in all of these networks, and we are quickly able to reduce the remaining search space when it isn't the largest $k$-core as well.

We observe several interesting properties in these temporal strong components. In the two contact networks (infect-hyper and infect-dublin), both of the largest strong components had about 100 vertices, despite the drastically different sizes of the initial dataset. We suspect this is a consequence of the data collection methodology since the infect-dublin data were collected over months whereas the infect-hyper data were collected over days.  In the interaction networks, the components contain a significant fraction of the total vertices, roughly 20-30\%.  In the retweet networks, the components are a much smaller fraction of the vertices.  
Given the strong communication pattern between the groups, the components are good candidates for centers communities in the networks. Finally, the hashtag networks have small temporal strong components; only a tiny fraction of the users participate in them.  

Together, these results show that temporal strong components are a strict requirement on a group of nodes in a network.  For instance, there is a considerable difference in the size of temporal strong components between networks with asymmetry in the relations (retweets and hashtags) compared with networks with symmetric relationships (fb-forum, fb-messages, and reality).  This finding may be important for those interested in designing seeded viral campaigns on these networks.






